Co-Decompositions and FO Model Checking

Tree decompositions describe large graphs as gluings of smaller component parts. Here we study their categorical duals, tree co-decompositions, which construct large graphs via fibered products of small constituent parts. Co-decompositions are compressed representations of graphs or relational structures: the decomposed object can be exponentially larger than the space required to specify the co-decomposition. Our main contribution is an algorithmic meta-theorem for first order logic: given only a co-decomposition of a $\sigma$-structure $G$ with $b$ bags, each of size at most $w$ and an FO sentence $\phi$, there is an algorithm which, without ever constructing or inspecting $G$, operates on the co-decomposition and determines whether $G \models \phi$ in time $f_\sigma(w,|\varphi|)\cdot b$. We pair this algorithm with structural results on tree co-width, including its relationship to tree-width and a separation from twin-width. Furthermore, we characterize bounded path co-width using a graph grammar. In contrast to our logical meta-theorem, we prove that $(s,t)$-Path becomes NP-hard on co-decomposition inputs. These results demonstrate how categorical constructions can enable efficient computation on exponentially compressed structures.

==> fig-lemma-atoms-in-bags.tex <==
% https://q.uiver.app/#q=WzAsMTAsWzAsMywiR18xIl0sWzIsMywiR197Mn0iXSxbMSw0LCJHX3sxLDJ9IixbMjcwLDYwLDQ3LDFdXSxbNCwzLCJHX3tiLTF9Il0sWzMsMywiXFxkb3RzIl0sWzYsMywiR197Yn0iXSxbNSw0LCJHX3tiLTEsIGJ9IixbMjcwLDYwLDQ3LDFdXSxbMywxLCJcXGxpbSBcXFBhIl0sWzMsMiwiXFxkb3RzIl0sWzMsMCwiW1xcZWxsXSJdLFswLDIsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFsxLDIsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFsxLDQsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFszLDYsIiIsMCx7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFs1LDYsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFszLDQsIiIsMix7InN0eWxlIjp7ImhlYWQiOnsibmFtZSI6ImVwaSJ9fX1dLFs3LDAsImdfezF9IiwxLHsiY29sb3VyIjpbMCw2MCw2MF19LFswLDYwLDYwLDFdXSxbNywxLCJnX3syfSIsMSx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzcsMywiZ197Yi0xfSIsMSx7ImNvbG91ciI6WzAsNjAsNjBdfSxbMCw2MCw2MCwxXV0sWzcsNSwiZ197Yn0iLDEseyJjb2xvdXIiOlswLDYwLDYwXX0sWzAsNjAsNjAsMV1dLFs5LDcsIlxcYmV0YSJdXQ==
    \begin{tikzcd}
	&&& {[\ell]} &&& \\
	&&& {\lim \Pa} \\
	&&& \dots \\
	{G_1} && {G_{2}} & \dots & {G_{b-1}} && {G_{b}} \\
	& \textcolor{rgb,255:red,120;green,48;blue,192}{{G_{1,2}}} &&&& \textcolor{rgb,255:red,120;green,48;blue,192}{{G_{b-1, b}}}
	\arrow["\beta", from=1-4, to=2-4]
	\arrow["{g_{1}}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=2-4, to=4-1]
	\arrow["{g_{2}}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=2-4, to=4-3]
	\arrow["{g_{b-1}}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=2-4, to=4-5]
	\arrow["{g_{b}}"{description}, color={rgb,255:red,214;green,92;blue,92}, from=2-4, to=4-7]
	\arrow[two heads, from=4-1, to=5-2]
	\arrow[two heads, from=4-3, to=4-4]
	\arrow[two heads, from=4-3, to=5-2]
	\arrow[two heads, from=4-5, to=4-4]
	\arrow[two heads, from=4-5, to=5-6]
	\arrow[two heads, from=4-7, to=5-6]
\end{tikzcd}
